Multiscale modeling of resistive switching in gold nanogranular films

Metallic nanogranular films display a complex dynamical response to a constant bias, showing up as atypical resistive switching mechanism which could be used to create electrical components for neuromorphic applications. To model such a phenomenon we use a multiscale approach blending together an ab initio treatment of the electric current at the nanoscale, a molecular dynamical approach dictating structural rearrangements, and a finite-element solution of the heat equation for heat propagation in the sample. We also consider structural changes due to electromigration which are modelled on the basis of experimental observations on similar systems. Within such an approach, we manage to describe some distinctive features of the resistive switching occurring in nanogranular film and provide a physical interpretation at the microscopic level.

==> EM_miquel.tex <==
After each ERN iteration, if the current through the ${ijk}$-th ERN element overcomes $I_{a,ijk}$ the associated effective cross-section, $A_{c,ijk}$ is virtually reduced by a factor $\beta$ and, according to \cite{lopez2021modeling}, this is accompanied by a change in its resistance value $R_{ijk}'=\beta R_{ijk}$ and a new couple of activation and failure current values, $I_{a,ijk}$ and $I_{d,ijk}$, to be used in the next ERN iteration. Note that we allow $A_{c,ijk}$ to be reduced down to $0.16$ nm$^2$ (corresponding to a minimal junction with area $a^2$, being $a$ the lattice constant of gold). We use $\beta=5$ to produce all the results in this work. Instead, if the the current overcomes the failure value, $I_{d,ijk}$, the junction breaks and no current is allowed to flow through that element anymore. Since the failure current of the $ijk$-th element, $I_{d,ijk}$, depends on the effective cross-section, $A_{c,ijk}$, and the latter in turn depends on whether $I_{a,ijk}$ has been reached, this describes a system that responds differently depending on the particular choices for $I_d$, $I_a$ (and their dependencies with $A_c$) as well as on how the system is polarized in time. We include this in the coarse grained ERN by giving to each element a precise couple of initial values, $(I_{a,ijk}^{(0)},I_{d,ijk}^{(0)})$.

With this we are able to qualitatively reproduce the curves in \cite{wu2007feedback} in which a polycrystalline Au nanowire $100$ nm wide and $200$ nm long ($7$ and $14$ ERN cells, respectively) is first activated under $0.15$ V to finally reach the electrical failure at $0.4$ V. The obtained curve for the related coarse-grained ERN is shown in Figure \ref{fig:fig3}: at low voltages, $V<0.05$ V, the sample displays a low resistance value ($R<$100 $\Omega$). At $V=0.1$ V some EM events occur (yellowish and bluish elements in the first pannel in Figure \ref{fig:fig3}) and, as a consequence, the sample becomes more resistive but still in the low resistance range ($<1$ k$\Omega$). At $V=0.2$ V EM events have brought the sample to a high resistive state ($10-100$ k$\Omega$) and some gaps can be identified as not colored grid elements in second to forth pannel. Further increasing of the voltage produce the failure of an important portion of the grid cells ending up with a short-circuited gold sample. Data shown in Figure \ref{fig:fig3} are obtained with $I_{a,i}^{(0)}$ and $I_{d,i}^{(0)}$ uniformly distributed between 19 $\mu$A to 23 $\mu$A and 32 $\mu$A and 38 $\mu$A, respectively. The $I_{a,i}^{(0)}$ values are chosen so that average current flowing through the sample just before the activation is in the order of magnitude of the measured one, i.e. $7$ mA. The upper limit for the $I_{d,i}^{(0)}$ range is set to be twice the lower limit for the $I_{a,i}^{(0)}$ one.

==> EM_walter.tex <==
In order to reproduce the three stages, for each cell we first define two thresholds,
$I_{i,s}$ and  $I_{i,f}$, with the following properties:
if the current flowing in the cell $I_i$ is lower than  $I_{i,s}$,
the \emph{shrinking} threshold, the cell resistance $R_i$ 
remains a constant $R_i=R_{i,0}$; 
if $I_i$ exceeds $I_{i,f}$, the \emph{failure} threshold, 
the cell resistance goes to infinity;
if $I_i$ is in between those two values, we say that the cell is in the shrinking regime
its resistance grows following an exponential law $R_i(I_i+\delta I)=\beta R_i(I_i)$
with $\beta>1$. For continuous variations of the current ($\delta I \to 0$)
this is encoded in the following function
\be\label{eq:RofI}
R_i(I_i)=R_{i,0}\left(
\frac{
1-\left(
1-e^{\alpha (I-I_{i,s})}
\right)\vartheta(I_i-I_{i,s})
}{
\vartheta(I_{i,f}-I_i)
}
\right)
\ee
where $R_{i,0}$ is the cell resistance at very low biases and the parameter 
$\alpha$ is a positive parameter determining the deterioration rate of the junction,
and for which $\alpha=(\beta-1)/\delta I$.\footnote{\walter{
The $\beta$ here defined is not the $\beta$ Miquel has introduced 
in previous versions of the manuscript.
I hope that this doesn't change things too much...
}}
Just like $R_{i,0}$, both thresholds change from cell to cell, 
but they are randomly picked from two well spaced ranges.
As one can see from Fig. \ref{fig:em}, by considering a grid.... 
and picking $R_{i,0}$ at random from ... and....
our simple model \eqref{eq:RofI} allows us to reproduce experimental results
with sufficient accuracy.

For a ng-film we consider the same function as in Eq. \eqref{eq:RofI},
with just two slight differences.
First, due to the high inhomogeneity within a single cell,
we consider a different Eq. \eqref{eq:RofI} for each direction $x,y,z$.
This accounts for the fact that inside a cell current can flow 
from a cluster to another not necessarily following a straight path 
along the direction of the external potential.
Second, we adapt the value used for $I_{i,s}$ andd $I_{f,s}$ 
using the empirical law $I_{f}=6\times 10^3  A_c^{0.425}$ \walter{well...}
not just to account for the differnt size of the cell
but also of the porosity that is present in cells representing a ng-film.
We therefore use an effective cross-section that is $0.3$ times the cell area
\walter{I completely made up that value,
but we could make an estimate somehow...},
reflecting the fact that electromigration will affect more
those regions inside a cell where the connection is poorer.

